Fast Zero-Shot Image Tagging

The well-known word analogy experiments show that the recent word vectors capture fine-grained linguistic regularities in words by linear vector offsets, but it is unclear how well the simple vector offsets can encode visual regularities over words. We study a particular image-word relevance relation in this paper. Our results show that the word vectors of relevant tags for a given image rank ahead of the irrelevant tags, along a principal direction in the word vector space. Inspired by this observation, we propose to solve image tagging by estimating the principal direction for an image. Particularly, we exploit linear mappings and nonlinear deep neural networks to approximate the principal direction from an input image. We arrive at a quite versatile tagging model. It runs fast given a test image, in constant time w.r.t.\ the training set size. It not only gives superior performance for the conventional tagging task on the NUS-WIDE dataset, but also outperforms competitive baselines on annotating images with previously unseen tags

==> baselines.tex <==
% !TEX root = main.tex
\section{Baselines}
\label{sBaselines}
Since the zero-shot tag ranking is a relatively new problem, in order to fully address the performance, we also proposed some baselines other than our main proposed method and state-of-art zero-shot learning techniques to comprehensively compare our method.

\subsection{Linear Regression}

Despite we consider estimating $f(\cdot)$ as a optimization problem in proposed method, an intuitive alternative would be considering it as a regression problem instead.

First we derive the image feature and rank-SVM hyperplane over seen tags for each image in the train set. Then we solved the regression between the hyperplane weights and image features in th training set in a closed form linear approach. After obtaining the linear mapping matrix between hyperplanes and image feature, we could map the image feature of given query image to its corresponding ranking hyperplane in the semantic space, thus derive its labeling confidence.

\subsection{Seen2Unssen}

Inspired by the fact that we could predict unseen tags from seen tags of same image as shown in the section~\ref{sRankability}, we developed a baseline which predicts unseen tags from the prediction confidence of seen tags generated in the state-of-art traditional tagging method.

The idea is to train a conventional tagging model on the seen tags training set first. And predict the confidence of seen tags on the testing image. After that we could obtain a unique label ranking list for each image based on their label confidences. Then for each image we train a rank-SVM in the embedding space based the ranking list as we did in section~\ref{sRankability}. Use the rank-SVM in the embedding space, we could obtain the confidence of unseen tags once we know their embeddings.

Please note that this is not a conventional tag completion task since the tag sets are disjoint despite both tasks are very similar.

\subsection{Akata+}
Since Akata \etal~\cite{akata_evaluation_2015} has achieved the state-of-art results in the zero-shot learning, it would be an appropriate baseline for us to compare. But since they are solving classification problem, they are enforcing dot product similarity between each image an each class in their objective function. So during our comparison, we duplicated the training samples with $n$ multiple labels into $n$ same images with different classes to simulate a multi-class scenario.

But that is not accurate and unfair to compare, hence we also extended their method to multi-label scenario and refer it as Akata+. In their loss function, they are maximizing the confidence difference between the only one positive tag and the maximum negative tag in each image during each iteration. And we are maximizing the confidence difference between the every positive tag and the maximum negative tag in each image during each iteration in order to directly optimize the multi-label problem.

\subsection{Linear Fast0Tag}

In the baseline, we are still solving the same optimization problem in the proposed method. But instead we are approximating $f(\cdot)$ using a linear mapping over image feature instead of a neural network.

==> disc.tex <==
% !TEX root = main_final.tex
\section{Discussion}
\label{sDiscussion}

At the first glimpse, our approach might appear similar with traditional zero-shot learning methods~\cite{akata_label-embedding_2013,frome_devise:_2013,weston_wsabie:_2011}, which adopted the decision function similar to eq.~(\ref{eDecisionRule}). Yet they have different underlying assumptions and methods when taken a closer look. An abstract yet proper analogy between them is rank SVM to nearest neighbor classifier. Their difference could be conclude as follow:

Conventional zero-shot classifiers are metric learning methods while { Fast\textbf{0}Tag } is not. They are learning a transformation so that x, a image representation after learned transformation, in eq.~(\ref{eDecisionRule}) would be as close as possible to its corresponding class embedding in either joint latent space or embedding space. Hence eq.~(\ref{eDecisionRule}) in their work is exactly mesuring the distance between x and other samples in cosine similarity. Since x in { Fast\textbf{0}Tag } is a direction in embedding sapce instead of transformed image representation, eq.~(\ref{eDecisionRule}) here is merely project the embedding onto the direction x.

{ Fast\textbf{0}Tag } is a ranking method utilizing tag correlation leveraged from the word embedding analogy property as described in introduction, while conventional zero-shot learning methods are nearest neighbor classifiers inherently unable to incorporate tag corelation from embedding analogy or any other means.






\eat{
\subsection{Difference with Other Zero-Shot Methods}
This section states the reason that current zero-shot classification method is not a optimal way to solve the zero-shot multi-labeling problem. And it also state the reason why we introduce the hyperplane to solve the multi-labeling problem. We also compare our method with the only known zero-shot labeling method~\cite{fu_transductive_2015}.

To the best of our knowledge, all the known label-embedding-based zero-shot classification method share some common assumptions. And one of those assumptions is that each instance in visual domain corresponds to one points in the label embedding space. This is a reasonable assumption in classification problem in which each instance has a certain label. But such assumption violates the definition of zero-shot multi-labeling problem, in which each visual instance is represented as one or more points in the label embedding space.

Under such case, the zero-shot classification problem tries to derive the projection $\mathbf{f}:x\rightarrow y$, where $x$ is an visual representation of image or video, and $y$ is its corresponding label embedding. If we follow the same assumption to solve the multi-labeling problem, it would become $\mathbf{f}:x\rightarrow Y$, where $Y$ is a set of label embeddings representing the image or video. In such case the projection is no longer well-defined and can not be derived efficiently.

One may argue that it is possible to use the ranking information from $\mathbf{f}:x\rightarrow y$ to rank the labels and solve the labeling problem. But in zero-shot classification, labels are ranked according to their distances to the predicted points in semantic space. In this case, the highly ranked labels will be synonyms of prediction. Hence it will not help predicting the semantically diverse labels in multi-labeling problem, which is also proven in the experiments.

We also want to discuss the difference between our method and the only known zero-shot labeling method~\cite{fu_transductive_2015}. It is too computational complex to apply this method on NUS dataset since it searches the power set of testing tags during prediction. It would generate $2^{81}$  testing candidates in the aforementioned zero-shot task. Even a binary vector with equivalent size would cost $10^{14}$ GB to store. Hence we did not include this method as one of our baselines.

\subsection{Computational Complexity Analysis}

We would also look into the training process of different method, which is a important performance metric. We put the comparison of computational complexity in table.~\ref{tbl:complexity}. Part of the data is from~\cite{li_socializing_2015}.

\begin{table*}
\tiny
\begin{center}
\begin{tabular}{|l||c c c c|}

\hline
{\bf Method} & {\bf Training Computation} & {\bf Testing Computation} & {\bf Training Memory} & {\bf Testing Memory} \\
\hline\hline

TagProp~\cite{guillaumin_tagprop:_2009} & $O(l\cdot A_{train}\cdot k+A_{train}^2\cdot D_v^2)$ & $O(A_{test}(D_v|S|+k\log|S|)+A_{test}^2\cdot D_v^2)$ & $O(A_{train}(D_v|S|+2A_{train}))$ & $O(n(D_v|S|+2A_{test}))$ \\
\hline
{\bf Ours} & $O(l\cdot A_{train}\cdot p)$ & $O(A_{test}/codt p)$ & $O(p+p \cdot b)$ & $O(p+p \cdot b)$ \\

\hline
\end{tabular}
\end{center}
\caption{Computational Complexity Comparison}
\label{tbl:complexity}
\end{table*}

In table.~\ref{tbl:complexity}, $l$ is the number of iterations, $k$ is the number of nearest neighbor, $p$ is the complexity of neural network and $b$ is the batch size of neural network.

}
